The Heterogeneous Productivity Effects of Generative AI

We analyse the individual productivity effects of Italy's ban on ChatGPT, a generative pretrained transformer chatbot. We compile data on the daily coding output quantity and quality of over 36,000 GitHub users in Italy and other European countries and combine these data with the sudden announcement of the ban in a difference-in-differences framework. Among the affected users in Italy, we find a short-term increase in output quantity and quality for less experienced users and a decrease in productivity on more routine tasks for experienced users.

==> _retired/did-table-poisson.tex <==
\begin{table}

\caption{Poisson pseudolikelihood regression}
\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}[t]{cccccccc}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{4}{c}{Output Quantity} & \multicolumn{1}{c}{PR complexity} \\
\cmidrule(l{3pt}r{3pt}){4-7} \cmidrule(l{3pt}r{3pt}){8-8}
\multicolumn{3}{c}{ } & \multicolumn{1}{c}{\makecell[c]{Events\\}} & \multicolumn{1}{c}{\makecell[c]{Output\\}} & \multicolumn{1}{c}{\makecell[c]{Releases\\}} & \multicolumn{1}{c}{\makecell[c]{PushPull\\}} & \multicolumn{1}{c}{\makecell[c]{Files changed\\ per PR}} \\
 &  &  & (1) & (2) & (3) & (4) & (5)\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textbf{Pre 27/28.03 - Post 03/04.04}}\\
\hspace{1em} & Users with Affiliation & Treat $\times$ Post & -0.0394 & -0.0631 & -0.3099 & -0.0758 & -1.8728***\\

\hspace{1em} &  &  & (0.0715) & (0.0741) & (0.2919) & (0.0747) & (0.5665)\\

\hspace{1em} &  & Post & 0.0990*** & 0.1074*** & 0.0067 & 0.1108*** & 1.2271***\\

\hspace{1em} &  &  & (0.0279) & (0.0288) & (0.1253) & (0.0319) & (0.3909)\\

\hspace{1em} &  & N & 16936 & 16304 & 1376 & 15420 & 7116\\
\cmidrule{2-8}
\hspace{1em} & Users w/o Affiliation & Treat $\times$ Post & 0.0376 & 0.0624 & -0.3470 & 0.0835 & 0.4111\\

\hspace{1em} &  &  & (0.0692) & (0.0723) & (0.3835) & (0.0812) & (1.0620)\\

\hspace{1em} &  & Post & 0.0156 & 0.0128 & -0.0494 & 0.0217 & -0.8816\\

\hspace{1em} &  &  & (0.0375) & (0.0385) & (0.1916) & (0.0432) & (0.7686)\\

\hspace{1em} &  & N & 12940 & 12320 & 752 & 11668 & 3652\\
\cmidrule{1-8}
\addlinespace[0.3em]
\multicolumn{8}{l}{\textbf{Pre 27/28/29.03 - Post 05/06/11.04}}\\
\hspace{1em} & Users with Affiliation & Treat $\times$ Post & 0.0231 & 0.0348 & -0.0703 & 0.0271 & -0.8982\\

\hspace{1em} &  &  & (0.0570) & (0.0574) & (0.2465) & (0.0599) & (0.7032)\\

\hspace{1em} &  & Post & -0.0021 & -0.0091 & -0.0334 & -0.0002 & -0.3873*\\

\hspace{1em} &  &  & (0.0234) & (0.0240) & (0.1150) & (0.0266) & (0.2218)\\

\hspace{1em} &  & N & 30982 & 30317 & 3353 & 29505 & 14560\\
\cmidrule{2-8}
\hspace{1em} & Users w/o Affiliation & Treat $\times$ Post & 0.0257 & 0.0211 & -0.2502 & 0.0248 & -0.0228\\

\hspace{1em} &  &  & (0.0589) & (0.0597) & (0.3283) & (0.0636) & (0.8388)\\

\hspace{1em} &  & Post & -0.0245 & -0.0364 & 0.1325 & -0.0299 & -1.0768*\\

\hspace{1em} &  &  & (0.0308) & (0.0311) & (0.1559) & (0.0340) & (0.6494)\\

\hspace{1em} &  & N & 24304 & 23394 & 1967 & 22659 & 7882\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \textit{Notes:} 
\item All specifications include user fixed effects. Robust standard errors are clustered on the user-level in parentheses: *p<0.1, ** p<0.5, *** p<0.01.
\end{tablenotes}
\end{threeparttable}}
\end{table}


==> _retired/did-table-v20230501.tex <==
%\begin{landscape}
\begin{table}[!h]
\caption{\label{tab:baseline}The Effect of the ChatGPT Ban on GitHub Output }
\centering
%\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}[t]{lcccccccc}
\toprule
&\multicolumn{4}{c}{ \textbf{Users with Affiliation}} &\multicolumn{4}{c}{\textbf{Users w/o Affiliation}}\\
&Events &  Release   &     Output  & PushPull & Events &  Release   &     Output  & PushPull     \\ 
\cline{2-9} 
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)   \\
\midrule
&\multicolumn{8}{c}{\textit{A: Pre 27/28.03 - Post 03/04.04}} \\ 
\cline{2-9} 

Treat$\times$Post&       0.115   &      -0.012** &      -0.278   &      -0.227   &       0.005   &      -0.003   &       0.188   &       0.192   \\
            &     (0.109)   &     (0.005)   &     (0.295)   &     (0.207)   &     (0.120)   &     (0.005)   &     (0.221)   &     (0.189)   \\
Post  &       0.052   &       0.002   &       0.453***&       0.323***&      -0.013   &       0.002   &       0.040   &       0.051   \\
            &     (0.053)   &     (0.002)   &     (0.123)   &     (0.094)   &     (0.060)   &     (0.002)   &     (0.119)   &     (0.101)   \\
\midrule
 
N           &   18332  &   18332    &   18332   &   18332   & 14496   &   14496   &   14496   &   14496   \\
\midrule
&\multicolumn{8}{c}{\textit{B: Pre 27/28/29.03 - Post 05/06/11.04}} \\ 
\cline{2-9} 


Treat$\times$Post&       0.048   &      -0.003   &       0.135   &       0.073   &       0.003   &       0.000   &       0.067   &       0.058   \\
            &     (0.090)   &     (0.004)   &     (0.223)   &     (0.163)   &     (0.101)   &     (0.004)   &     (0.175)   &     (0.142)   \\
Post &      -0.217***&      -0.002   &      -0.037   &      -0.001   &      -0.325***&      -0.000   &      -0.112   &      -0.069   \\
            &     (0.042)   &     (0.002)   &     (0.097)   &     (0.074)   &     (0.050)   &     (0.002)   &     (0.095)   &     (0.078)   \\\midrule

N           &   31983   &   31983   &   31983   &   31983   &   25368   &   25368  &   25368  &   25368  \\
 
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item \textit{Notes:} 
\item All specifications include user fixed effects. Robust standard errors are clustered on the user-level in parentheses: *p<0.1, ** p<0.5, *** p<0.01.
\end{tablenotes}
\end{threeparttable}
\end{table}
%\end{landscape}
